CLASH: Complementary Learning with Neural Architecture Search for Gait Recognition

Gait recognition, which aims at identifying individuals by their walking patterns, has achieved great success based on silhouette. The binary silhouette sequence encodes the walking pattern within the sparse boundary representation. Therefore, most pixels in the silhouette are under-sensitive to the walking pattern since the sparse boundary lacks dense spatial-temporal information, which is suitable to be represented with dense texture. To enhance the sensitivity to the walking pattern while maintaining the robustness of recognition, we present a Complementary Learning with neural Architecture Search (CLASH) framework, consisting of walking pattern sensitive gait descriptor named dense spatial-temporal field (DSTF) and neural architecture search based complementary learning (NCL). Specifically, DSTF transforms the representation from the sparse binary boundary into the dense distance-based texture, which is sensitive to the walking pattern at the pixel level. Further, NCL presents a task-specific search space for complementary learning, which mutually complements the sensitivity of DSTF and the robustness of the silhouette to represent the walking pattern effectively. Extensive experiments demonstrate the effectiveness of the proposed methods under both in-the-lab and in-the-wild scenarios. On CASIA-B, we achieve rank-1 accuracy of 98.8%, 96.5%, and 89.3% under three conditions. On OU-MVLP, we achieve rank-1 accuracy of 91.9%. Under the latest in-the-wild datasets, we outperform the latest silhouette-based methods by 16.3% and 19.7% on Gait3D and GREW, respectively.

==> table/arch.tex <==
\begin{table}[t]
    \caption{Ablation study for the architecture of the feature extractor w/o  and w/ weight-sharing strategy.}
    \small
    \centering
    \renewcommand{\arraystretch}{0.85}
    \scalebox{1}[1]{
    \begin{tabular}{c|ccc|c}
    \toprule
    Methods               & NM & BG & CL & Mean \\
    \midrule
    Baseline              &  96.5 & 93.1 &82.7 &90.8      \\
    Ours w/o Share &    97.7 &94.5& 86.5& 92.9      \\
   \textbf{Ours (w/ Share)}           &   \textbf{98.0}  & \textbf{95.2}   & \textbf{87.0}   &  \textbf{93.4}    \\ \bottomrule
    \end{tabular}}
    \label{tab:share}
    \end{table}



==> table/casia.tex <==
\begin{table*}[t]
    \centering
    \footnotesize

    
    \caption{Averaged rank-1 accuracy on CASIA-B under LT setting, excluding identical views cases.}
    % , including GaitSet~\cite{chao2019gaitset}, GaitPart~\cite{Fan_2020_CVPR}, GLN~\cite{hou2020gait}, MT3D~\cite{lin2020gait}, CSTL~\cite{Huang_2021_ICCV}, 3DLocal~\cite{Huang_2021_ICCV2}, and GaitGL~\cite{Lin_2021_ICCV}
    \renewcommand{\arraystretch}{0.85}
    \scalebox{1}[1]{
    \begin{tabular}{l|c|c|ccccccccccc|c}
    \toprule  
    \multicolumn{3}{l|}{Gallery NM \#1-4}                             & \multicolumn{11}{c|}{0$^{\circ}$-180$^{\circ}$}                                                & \multirow{2}{*}{Mean} \\ \cmidrule{1-14}
    Probe                & \multicolumn{1}{l|}{Resolution} & Method   & 0$^{\circ}$    & 18$^{\circ}$   & 36$^{\circ}$   & 54$^{\circ}$   & 72$^{\circ}$   & 90$^{\circ}$   & 108$^{\circ}$  & 126$^{\circ}$  & 144$^{\circ}$  & 162$^{\circ}$  & 180$^{\circ}$  &                       \\ \midrule
    \multirow{12}{*}{NM} &  \multirow{7}{*}{$64 \times 44$}          & GaitSet~\cite{chao2019gaitset}  & 90.8 & 97.9 & 99.4 & 96.9 & 93.6 & 91.7 & 95.0 & 97.8 & 98.9 & 96.8 & 85.8 & 95.0                  \\  
                         &                                 & GaitPart~\cite{Fan_2020_CVPR} & 94.1 & 98.6 & 99.3 & 98.5 & 94.0 & 92.3 & 95.9 & 98.4 & 99.2 & 97.8 & 90.4 & 96.2                  \\  
                         &                                 & MT3D~\cite{lin2020gait}     & 95.7 & 98.2 & 99.0 & 97.5 & 95.1 & 93.9 & 96.1 & 98.6 & 99.2 & 98.2 & 92.0 & 96.7                  \\  
                         &                                 & CSTL~\cite{Huang_2021_ICCV}     & 97.2 & 99.0 & 99.2 & 98.1 & 96.2 & 95.5 & 97.7 & 98.7 & 99.2 & 98.9 & \textbf{96.5} & 97.8                  \\  
                         &                                 & 3DLocal~\cite{Huang_2021_ICCV2}  & 96.0 & 99.0 & 99.5 & 98.9 & 97.1 & 94.2 & 96.3 & \textbf{99.0} & 98.8 & 98.5 & 95.2 & 97.5                  \\  
                         &                                 & GaitGL~\cite{Lin_2021_ICCV}   &      96.0 &98.3& 99.0& 97.9& 96.9 &95.4& 97.0& 98.9& 99.3& 98.8& 94.0& 97.4                      \\  
                         &                                 & \textbf{Ours}     & \textbf{97.2}&\textbf{99.2}&\textbf{99.5}&\textbf{99.1}&\textbf{97.2}&\textbf{95.7}&\textbf{98.0}&98.9&\textbf{99.3}&
                         \textbf{99.1}&96.3&\textbf{98.1}  \\ \cline{2-15} 
                         & \multirow{5}{*}{$128 \times 88$}        &   GaitSet  & 91.4 & 98.5 & 98.8 & 97.2 & 94.8 & 92.9 & 95.4 & 97.9 & 98.8 & 96.5 & 89.1 & 95.6                  \\  
                         &                                 &   GLN~\cite{hou2020gait}      & 93.2 & 99.3 & 99.5 & 98.7 & 96.1 & 95.6 & 97.2 & 98.1 & 99.3 & 98.6 & 90.1 & 96.9                  \\  
                         &                                 &   CSTL     & 97.8 & 99.4 & 99.2 & 98.4 & 97.3 & 95.2 & 96.7 & 98.9 & 99.4 & 99.3 & 96.7 & 98.0                  \\  
                         &                                 &   3DLocal  & 97.8 & 99.4 & 99.7 & 99.3 & 97.5 & 96.0 & 98.3 & 99.1 & \textbf{99.9} & 99.2 & 94.6 & 98.3                  \\  
                         &                                 &  \textbf{Ours}     &   \textbf{98.1}&\textbf{99.5}&\textbf{99.7}&\textbf{99.5}&\textbf{97.8}&\textbf{96.7}&\textbf{98.8}&\textbf{99.3}&99.7&\textbf{99.5}&\textbf{97.4}&\textbf{98.7}               \\ \hline
    \multirow{12}{*}{BG} & \multirow{7}{*}{$64 \times 44$}          & GaitSet  & 83.8 & 91.2 & 91.8 & 88.8 & 83.3 & 81.0 & 84.1 & 90.0 & 92.2 & 94.4 & 79.0 & 87.2                  \\  
                         &                                 & GaitPart & 89.1 & 94.8 & 96.7 & 95.1 & 88.3 & 84.9 & 89.0 & 93.5 & 96.1 & 93.8 & 85.8 & 91.5                  \\  
                         &                                 & MT3D     & 91.0 & 95.4 & 97.5 & 94.2 & 92.3 & 86.9 & 91.2 & 95.6 & 97.3 & 96.4 & 86.6 & 93.0                  \\  
                         &                                 & CSTL     & 91.7 & 96.5 & 97.0 & 95.4 & 90.9 & 88.0 & 91.5 & 95.8 & 97.0 & 95.5 & 90.3 & 93.6                  \\  
                         &                                 & 3DLocal  & 92.9 & 95.9 & 97.8 & 96.2 & 93.0 & 87.8 & 92.7 & 96.3 & 97.9 & 98.0 & 88.5 & 94.3                  \\  
                         &                                 & GaitGL   &    92.6 &96.6& 96.8 &95.5& 93.5& 89.3& 92.2& 96.5& 98.2& 96.9& 91.5& 94.5                   \\  
                         &                                 & \textbf{Ours}     &   \textbf{93.0}&\textbf{96.8}&\textbf{97.9}&\textbf{96.5}&\textbf{94.5}&\textbf{90.1}&\textbf{93.0}&\textbf{97.2}&\textbf{98.8}&
                         \textbf{98.2}&\textbf{92.2}&\textbf{95.3}              \\ \cline{2-15} 
                         & \multirow{5}{*}{$128 \times 88$}        &   GaitSet  & 89.0 & 95.3 & 95.6 & 94.0 & 89.7 & 86.7 & 89.7 & 94.3 & 95.4 & 92.7 & 84.4 & 91.5                  \\  
                         &                                 &   GLN      & 91.1 & 97.7 & 97.8 & 95.2 & 92.5 & 91.2 & 92.4 & 96.0 & 97.5 & 95.0 & 88.1 & 94.0                  \\  
                         &                                 &   CSTL     & 95.0 & 96.8 & 97.9 & 96.0 & 94.0 & 90.5 & 92.5 & 96.8 & 97.9 & 99.0 & \textbf{94.3} & 95.4                  \\  
                         &                                 &   3DLocal  & 94.7 & 98.7 & 98.8 & 97.5 & 93.3 & 91.7 & 92.8 & 96.5 & 98.1 & 97.3 & 90.7 & 95.5                  \\  
                         &                                 &   \textbf{Ours}     &  \textbf{95.2}&\textbf{98.8}&\textbf{99.4}&\textbf{98.2}&\textbf{94.1}&\textbf{92.4}&\textbf{93.3}&\textbf{96.9}&
                         \textbf{98.4}&\textbf{99.1}&93.8&\textbf{96.3}          \\ \hline
    \multirow{12}{*}{CL} & \multirow{7}{*}{$64 \times 44$}          & GaitSet  & 61.4 & 75.4 & 80.7 & 77.3 & 72.1 & 70.1 & 71.5 & 73.5 & 73.5 & 68.4 & 50.0 & 70.4                  \\  
                         &                                 & GaitPart & 70.7 & 85.5 & 86.9 & 83.3 & 77.1 & 72.5 & 76.9 & 82.2 & 83.8 & 80.2 & 66.5 & 78.7                  \\  
                         &                                 & MT3D     & 76.0 & 87.6 & 89.8 & 85.0 & 81.2 & 75.7 & 81.0 & 84.5 & 85.4 & 82.2 & 68.1 & 81.5                  \\  
                         &                                 & CSTL     & 78.1 & 89.4 & 91.6 & 86.6 & 82.1 & 79.9 & 81.8 & 86.3 & 88.7 & 86.6 & 75.3 & 84.2                  \\  
                         &                                 & 3DLocal  & 78.2 & 90.2 & 92.0 & 87.1 & 83.0 & 76.8 & 83.1 & 86.6 & 86.8 & 84.1 & 70.9 & 83.7                  \\  
                         &                                 & GaitGL   &     76.6& 90.0& 90.3& 87.1& 84.5& 79.0& 84.1& 87.0& 87.3& 84.4& 69.5& 83.6                   \\  
                         &                                 & \textbf{Ours}     & \textbf{80.2}&\textbf{91.9}&\textbf{93.1}&\textbf{88.4}&\textbf{86.5}&\textbf{83.3}&\textbf{84.6}&\textbf{90.3}&\textbf{91.0}&\textbf{88.8}&\textbf{78.4}&\textbf{87.0}          \\ \cline{2-15} 
                         & \multirow{5}{*}{$128 \times 88$}        &  GaitSet  & 66.3 & 79.4 & 84.5 & 80.7 & 74.6 & 73.2 & 74.1 & 80.3 & 79.7 & 72.3 & 62.9 & 75.3                  \\  
                         &                                 &  GLN      & 70.6 & 82.4 & 85.2 & 82.7 & 79.2 & 76.4 & 76.2 & 78.9 & 77.9 & 78.7 & 64.3 & 77.5                  \\  
                         &                                 &    CSTL     & 84.1 & 92.1 & 91.8 & 87.2 & 84.4 & 81.5 & 84.5 & 88.4 & 91.6 & 91.2 & 79.9 & 87.0                  \\  
                         &                                 &   3DLocal  & 78.5 & 88.9 & 91.0 & 89.2 & 83.7 & 80.5 & 83.2 & 84.3 & 87.9 & 87.1 & 74.7 & 84.5                  \\  
                         &                                 &   \textbf{Ours}     &    \textbf{87.3}&\textbf{94.6}&\textbf{93.0}&\textbf{89.9}&\textbf{86.4}&\textbf{83.9}&\textbf{86.7}&\textbf{89.2}&\textbf{93.8}&\textbf{93.1}&\textbf{81.3}&\textbf{89.0}  \\ \bottomrule          
    \end{tabular}}
    \label{tab:casia}
    \end{table*}


    


==> table/cell.tex <==
\begin{table}[t]
    \centering
   \small
    \caption{Ablation study for our task-specific search space. }
    % The combinations of MD cell and MT cell are presented below.  }
      \renewcommand{\arraystretch}{0.75}
    \scalebox{1}[1]{
    \begin{tabular}{c|c|ccc|c}
    \toprule
    \multicolumn{2}{c|}{Method} &
      \multicolumn{1}{c}{\multirow{2}{*}{NM}} &
      \multicolumn{1}{c}{\multirow{2}{*}{BG}} &
      \multicolumn{1}{c|}{\multirow{2}{*}{CL}} &
      \multicolumn{1}{c}{\multirow{2}{*}{Mean}} \\ \cmidrule{1-2}
    \multicolumn{1}{c|}{MT Cell} &
      \multicolumn{1}{c|}{MD Cell} &
      \multicolumn{1}{c}{} &
      \multicolumn{1}{c}{} &
      \multicolumn{1}{c|}{} &
      \multicolumn{1}{c}{} \\
      \midrule
     &                          & 97.0 & 92.1 &82.0 &90.8 \\ 
     \checkmark&                & 97.4 &  93.0 &  84.2 & 91.5 \\ 
     & \checkmark              & 97.7  & 95.0 & 86.4 & 93.0  \\ 
     \checkmark& \checkmark     & \textbf{98.1} & \textbf{95.3} & \textbf{87.0} & \textbf{93.5}  \\

     \bottomrule
    \end{tabular}}
    \label{tab:cell}
    \end{table}
    
    
    
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


==> table/stdf.tex <==




\begin{table}[t]
\caption{Effectiveness of Bi-DT, foreground/background separation (F/B Sep.), and NCL. Naive Fuser is a 3D CNN with about equal parameters as the searched MD cell for fairness.}
\centering
\small
\renewcommand{\arraystretch}{0.85}
% \renewcommand{\arraystretch}{0.85}
\begin{tabular}{cl|cccc}
\toprule
\multicolumn{2}{c|}{Method}                                        & NM                   & BG                   & CL                   & Mean                 \\ \midrule
\multicolumn{1}{l|}{\multirow{4}{*}{DSTF}} & Baseline w/ NCL         &  96.5                    &        91.6              &       82.4               &  90.2                    \\
\multicolumn{ 1}{l|}{}                      & \hspace{1em}+Bi-DT                     &     97.2                 &    93.7                  &        84.4              &     91.8                 \\
\multicolumn{1}{l|}{}                      &  \hspace{1em}+ Bi-DT+ F/B Sep.                    &          97.3 & 94.1 & 85.3 & 92.2                  \\ \midrule
\multicolumn{1}{l|}{\multirow{4}{*}{NCL}}  &  Baseline w/ DSTF                    & 97.4                      &       93.0               &   84.2                   &  91.5                    \\
\multicolumn{1}{l|}{}                      &\hspace{1em}+ MT  & 97.3 & 94.1 & 85.3 & 92.2  \\
\multicolumn{1}{l|}{}                      &\hspace{1em}+ MT + Naive Fuser  & 97.3 & 94.1 & 85.3 & 92.2  \\
\multicolumn{1}{l|}{}                      &\hspace{1em}+ NCL (MT + MD)  & \textbf{98.1} & \textbf{95.3} &  \textbf{87.0} &\textbf{93.5}  \\ \bottomrule
\end{tabular}
\label{tab:analyse}
\end{table}

==> table/stream.tex <==
\begin{table}[t]
\caption{Ablation study for different combinations of descriptors. `Sil' and `Sil-D' denotes the silhouette and silhouette with inter-frame difference, respectively.}
\small
\centering
  \renewcommand{\arraystretch}{0.8}
\begin{tabular}{c|c|ccc|c}
\toprule
Stream A & Stream B & NM & BG & CL & Mean \\ \midrule
Sil      & Sil      & 96.8 & 93.8& 85.3& 91.9    \\
Sil      & Sil-D    &   94.8 &  92.6  & 80.1   &  89.1    \\
STAF       & STAF       &  95.0  &   90.2 &   75.8 &  87.0    \\
Sil      &    Bi-DT   &  97.7 & 94.6& 86.1& 92.8     \\
\textbf{Sil}      & \textbf{STAF}    &  \textbf{98.0}  & \textbf{95.2}   & \textbf{87.0}   &  \textbf{93.4}    \\
\bottomrule
\end{tabular}
\end{table}


